V-MPO: On-Policy Maximum a Posteriori Policy Optimization for Discrete and Continuous Control

Some of the most successful applications of deep reinforcement learning to challenging domains in discrete and continuous control have used policy gradient methods in the on-policy setting. However, policy gradients can suffer from large variance that may limit performance, and in practice require carefully tuned entropy regularization to prevent policy collapse. As an alternative to policy gradient algorithms, we introduce V-MPO, an on-policy adaptation of Maximum a Posteriori Policy Optimization (MPO) that performs policy iteration based on a learned state-value function. We show that V-MPO surpasses previously reported scores for both the Atari-57 and DMLab-30 benchmark suites in the multi-task setting, and does so reliably without importance weighting, entropy regularization, or population-based tuning of hyperparameters. On individual DMLab and Atari levels, the proposed algorithm can achieve scores that are substantially higher than has previously been reported. V-MPO is also applicable to problems with high-dimensional, continuous action spaces, which we demonstrate in the context of learning to control simulated humanoids with 22 degrees of freedom from full state observations and 56 degrees of freedom from pixel observations, as well as example OpenAI Gym tasks where V-MPO achieves substantially higher asymptotic scores than previously reported.

==> V-MPO arXiv/atari57_scores.tex <==
% max_environment_steps = 11.4B
% num_recent = 10
alien               &    1163.00 $\pm$     148.43 &    2332.00 $\pm$     290.16&      13.55 $\pm$       2.15 &      30.50 $\pm$       4.21 \\
amidar              &     192.50 $\pm$       9.16 &     423.60 $\pm$      20.53&      10.89 $\pm$       0.53 &      24.38 $\pm$       1.20 \\
assault             &    4215.30 $\pm$     294.51 &    1225.90 $\pm$      60.64&     768.46 $\pm$      56.68 &     193.13 $\pm$      11.67 \\
asterix             &    4180.00 $\pm$     303.91 &    9955.00 $\pm$    2043.48&      47.87 $\pm$       3.66 &     117.50 $\pm$      24.64 \\
asteroids           &    3473.00 $\pm$     381.30 &    2982.00 $\pm$     164.35&       5.90 $\pm$       0.82 &       4.85 $\pm$       0.35 \\
atlantis            &  997530.00 $\pm$    3552.89 &  940310.00 $\pm$    6085.96&    6086.50 $\pm$      21.96 &    5732.81 $\pm$      37.62 \\
bank\_heist         &    1329.00 $\pm$       2.21 &    1563.00 $\pm$      15.81&     177.94 $\pm$       0.30 &     209.61 $\pm$       2.14 \\
battle\_zone        &   43900.00 $\pm$    4738.04 &   61400.00 $\pm$    5958.52&     119.27 $\pm$      13.60 &     169.52 $\pm$      17.11 \\
beam\_rider         &    4598.00 $\pm$     618.09 &    3868.20 $\pm$     666.55&      25.56 $\pm$       3.73 &      21.16 $\pm$       4.02 \\
berzerk             &    1018.00 $\pm$      72.63 &    1424.00 $\pm$     150.93&      35.68 $\pm$       2.90 &      51.87 $\pm$       6.02 \\
bowling             &      63.60 $\pm$       0.84 &      27.60 $\pm$       0.62&      29.43 $\pm$       0.61 &       3.27 $\pm$       0.45 \\
boxing              &      93.10 $\pm$       0.94 &     100.00 $\pm$       0.00&     775.00 $\pm$       7.86 &     832.50 $\pm$       0.00 \\
breakout            &     484.30 $\pm$      57.24 &     400.70 $\pm$      18.82&    1675.69 $\pm$     198.77 &    1385.42 $\pm$      65.36 \\
centipede           &    6037.90 $\pm$     994.99 &    3015.00 $\pm$     404.97&      39.76 $\pm$      10.02 &       9.31 $\pm$       4.08 \\
chopper\_command    &    4250.00 $\pm$     417.91 &    4340.00 $\pm$     714.45&      52.29 $\pm$       6.35 &      53.66 $\pm$      10.86 \\
crazy\_climber      &  100440.00 $\pm$    9421.56 &  116760.00 $\pm$    5312.12&     357.94 $\pm$      37.61 &     423.09 $\pm$      21.21 \\
defender            &   41585.00 $\pm$    4194.42 &   98395.00 $\pm$   17552.17&     244.78 $\pm$      26.52 &     604.01 $\pm$     110.99 \\
demon\_attack       &   77880.00 $\pm$    8798.44 &   20243.00 $\pm$    5434.41&    4273.35 $\pm$     483.72 &    1104.56 $\pm$     298.77 \\
double\_dunk        &      -0.80 $\pm$       0.31 &      12.60 $\pm$       1.94&     809.09 $\pm$      14.08 &    1418.18 $\pm$      88.19 \\
enduro              &    1187.90 $\pm$      76.10 &    1453.80 $\pm$     104.37&     138.05 $\pm$       8.84 &     168.95 $\pm$      12.13 \\
fishing\_derby      &      21.60 $\pm$       3.46 &      33.80 $\pm$       2.10&     213.77 $\pm$       6.54 &     236.79 $\pm$       3.96 \\
freeway             &      32.10 $\pm$       0.17 &      33.20 $\pm$       0.28&     108.45 $\pm$       0.58 &     112.16 $\pm$       0.93 \\
frostbite           &     250.00 $\pm$       0.00 &     260.00 $\pm$       0.00&       4.33 $\pm$       0.00 &       4.56 $\pm$       0.00 \\
gopher              &   11720.00 $\pm$    1687.71 &    7576.00 $\pm$     973.13&     531.92 $\pm$      78.32 &     339.62 $\pm$      45.16 \\
gravitar            &    1095.00 $\pm$     232.75 &    3125.00 $\pm$     191.87&      29.01 $\pm$       7.32 &      92.88 $\pm$       6.04 \\
hero                &   13159.50 $\pm$      68.90 &   29196.50 $\pm$     752.06&      40.71 $\pm$       0.23 &      94.53 $\pm$       2.52 \\
ice\_hockey         &       4.80 $\pm$       1.31 &      10.60 $\pm$       2.00&     132.23 $\pm$      10.83 &     180.17 $\pm$      16.50 \\
jamesbond           &    1015.00 $\pm$      91.39 &    3805.00 $\pm$     595.92&     360.12 $\pm$      33.38 &    1379.11 $\pm$     217.65 \\
kangaroo            &    1780.00 $\pm$      18.97 &   12790.00 $\pm$     629.52&      57.93 $\pm$       0.64 &     427.02 $\pm$      21.10 \\
krull               &    9738.00 $\pm$     360.95 &    7359.00 $\pm$    1064.84&     762.53 $\pm$      33.81 &     539.67 $\pm$      99.75 \\
kung\_fu\_master    &   44340.00 $\pm$    2898.70 &   38620.00 $\pm$    2346.48&     196.11 $\pm$      12.90 &     170.66 $\pm$      10.44 \\
montezuma\_revenge  &       0.00 $\pm$       0.00 &       0.00 $\pm$       0.00&       0.00 $\pm$       0.00 &       0.00 $\pm$       0.00 \\
ms\_pacman          &    1953.00 $\pm$     227.12 &    2856.00 $\pm$     324.54&      24.77 $\pm$       3.42 &      38.36 $\pm$       4.88 \\
name\_this\_game    &    5708.00 $\pm$     354.92 &    9295.00 $\pm$     679.83&      59.33 $\pm$       6.17 &     121.64 $\pm$      11.81 \\
phoenix             &   37030.00 $\pm$    6415.95 &   19560.00 $\pm$    1843.44&     559.60 $\pm$      98.99 &     290.05 $\pm$      28.44 \\
pitfall             &      -4.90 $\pm$       2.34 &      -2.80 $\pm$       1.40&       3.35 $\pm$       0.04 &       3.39 $\pm$       0.02 \\
pong                &      20.80 $\pm$       0.19 &      21.00 $\pm$       0.00&     117.56 $\pm$       0.54 &     118.13 $\pm$       0.00 \\
private\_eye        &     100.00 $\pm$       0.00 &     100.00 $\pm$       0.00&       0.11 $\pm$       0.00 &       0.11 $\pm$       0.00 \\
qbert               &    5512.50 $\pm$     741.08 &   15297.50 $\pm$    1244.47&      40.24 $\pm$       5.58 &     113.86 $\pm$       9.36 \\
riverraid           &    8237.00 $\pm$      97.09 &   11160.00 $\pm$     733.06&      43.72 $\pm$       0.62 &      62.24 $\pm$       4.65 \\
road\_runner        &   28440.00 $\pm$    1215.99 &   51060.00 $\pm$    1560.72&     362.91 $\pm$      15.52 &     651.67 $\pm$      19.92 \\
robotank            &      29.60 $\pm$       2.15 &      46.80 $\pm$       3.42&     282.47 $\pm$      22.22 &     459.79 $\pm$      35.29 \\
seaquest            &    1888.00 $\pm$      63.26 &    9953.00 $\pm$     973.02&       4.33 $\pm$       0.15 &      23.54 $\pm$       2.32 \\
skiing              &  -16244.00 $\pm$     592.28 &  -15438.10 $\pm$    1573.39&       6.69 $\pm$       4.64 &      13.01 $\pm$      12.33 \\
solaris             &    1794.00 $\pm$     279.04 &    2194.00 $\pm$     417.91&       5.03 $\pm$       2.52 &       8.64 $\pm$       3.77 \\
space\_invaders     &     793.50 $\pm$      90.61 &    1771.50 $\pm$     201.95&      42.45 $\pm$       5.96 &     106.76 $\pm$      13.28 \\
star\_gunner        &   44860.00 $\pm$    5157.74 &   60120.00 $\pm$    1953.60&     461.05 $\pm$      53.80 &     620.24 $\pm$      20.38 \\
surround            &       2.50 $\pm$       1.04 &       4.00 $\pm$       0.62&      75.76 $\pm$       6.31 &      84.85 $\pm$       3.74 \\
tennis              &      -0.10 $\pm$       0.09 &      23.10 $\pm$       0.26&     152.90 $\pm$       0.61 &     302.58 $\pm$       1.69 \\
time\_pilot         &   10890.00 $\pm$     787.46 &   22330.00 $\pm$    2443.11&     440.77 $\pm$      47.40 &    1129.42 $\pm$     147.07 \\
tutankham           &     218.50 $\pm$      13.53 &     254.60 $\pm$       9.99&     132.59 $\pm$       8.66 &     155.70 $\pm$       6.40 \\
up\_n\_down         &  175083.00 $\pm$   16341.05 &   82913.00 $\pm$   12142.08&    1564.09 $\pm$     146.43 &     738.18 $\pm$     108.80 \\
venture             &       0.00 $\pm$       0.00 &       0.00 $\pm$       0.00&       0.00 $\pm$       0.00 &       0.00 $\pm$       0.00 \\
video\_pinball      &   59898.40 $\pm$   23875.14 &  198845.20 $\pm$   98768.54&     339.02 $\pm$     135.13 &    1125.46 $\pm$     559.03 \\
wizard\_of\_wor     &    6960.00 $\pm$    1730.97 &    7890.00 $\pm$    1595.77&     152.55 $\pm$      41.28 &     174.73 $\pm$      38.06 \\
yars\_revenge       &   12825.70 $\pm$    2065.90 &   41271.70 $\pm$    4726.72&      18.90 $\pm$       4.01 &      74.16 $\pm$       9.18 \\
zaxxon              &   11520.00 $\pm$     646.81 &   18820.00 $\pm$     754.69&     125.67 $\pm$       7.08 &     205.53 $\pm$       8.26 \\
\midrule
Median & & &     117.56 &     155.70 \\

==> V-MPO arXiv/content_abstract.tex <==
Some of the most successful applications of deep reinforcement learning to challenging domains in discrete and continuous control have used policy gradient methods in the on-policy setting. However, policy gradients can suffer from large variance that may limit performance, and in practice require carefully tuned entropy regularization to prevent policy collapse. As an alternative to policy gradient algorithms, we introduce V-MPO, an on-policy adaptation of Maximum a Posteriori Policy Optimization (MPO) that performs policy iteration based on a learned state-value function. We show that V-MPO surpasses previously reported scores for both the Atari-57 and DMLab-30 benchmark suites in the multi-task setting, and does so reliably without importance weighting, entropy regularization, or population-based tuning of hyperparameters. On individual DMLab and Atari levels, the proposed algorithm can achieve scores that are substantially higher than has previously been reported. V-MPO is also applicable to problems with high-dimensional, continuous action spaces, which we demonstrate in the context of learning to control simulated humanoids with 22 degrees of freedom from full state observations and 56 degrees of freedom from pixel observations, as well as example OpenAI Gym tasks where V-MPO achieves substantially higher asymptotic scores than previously reported.

==> V-MPO arXiv/content_acknowledgments.tex <==
\subsubsection*{Acknowledgments}
We thank Lorenzo Blanco, Trevor Cai, Greg Wayne, Chloe Hillier, and Vicky Langston for their assistance and support.

==> V-MPO arXiv/content_background.tex <==
\section{Background and setting}

We consider the discounted RL setting, where we seek to optimize a policy $\pi$ for a Markov Decision Process described by states $s$, actions $a$, initial state distribution $\rho_0^\text{env}(s_0)$, transition probabilities $\mathcal{P}^\text{env}(s_{t+1}|s_t,a_t)$, reward function $r(s_t,a_t)$, and discount factor $\gamma \in (0, 1)$. In deep RL, the policy $\pi_\theta(a_t|s_t)$, which specifies the probability that the agent takes action $a_t$ in state $s_t$ at time $t$, is described by a neural network with parameters $\theta$. We consider problems where both the states $s$ and actions $a$ may be discrete or continuous. Two functions play a central role in RL: the state-value function $V^\pi(s_t) = \mathbb{E}_{a_t,s_{t+1},a_{t+1},\ldots} \big[ \sum_{k=0}^\infty \gamma^k r(s_{t+k},a_{t+k}) \big]$ and the state-action value function $Q^\pi(s_t, a_t) = \mathbb{E}_{s_{t+1},a_{t+1},\ldots} \big[ \sum_{k=0}^\infty \gamma^k r(s_{t+k},a_{t+k}) \big] = r(s_t, a_t) + \gamma \mathbb{E}_{s_{t+1}} \big[ V^\pi(s_{t+1}) \big]$, where $s_0 \sim \rho_0^\text{env}(s_0)$, $a_t \sim \pi(a_t|s_t)$, and $s_{t+1}\sim \mathcal{P}^\text{env}(s_{t+1}|s_t,a_t)$.

In the usual formulation of the RL problem, the goal is to find a policy $\pi$ that maximizes the expected return given by $J(\pi) = \mathbb{E}_{s_0,a_0,s_1,a_1,\ldots} \big[ \sum_{t=0}^\infty \gamma^t r(s_t,a_t) \big]$. In policy gradient algorithms~\cite{Williams1992,Sutton2000,Mnih2016}, for example, this objective is directly optimized by estimating the gradient of the expected return. An alternative approach to finding optimal policies derives from research that treats RL as a problem in probabilistic inference, including Maximum a Posteriori Policy Optimization (MPO)~\cite{Levine2018,Abdolmaleki2018a,Abdolmaleki2018}. Here our objective is subtly different, namely, given a suitable criterion for what are good actions to take in a certain state, how do we find a policy that achieves this goal?

As was the case for the original MPO algorithm, the following derivation is valid for any such criterion. However, the \emph{policy improvement theorem}~\cite{Sutton1998} tells us that a policy update performed by exact policy iteration, $\pi(s) = \argmax{a} [Q^\pi(s, a) - V^\pi(s)]$, can improve the policy if there is at least one state-action pair with a positive advantage and nonzero probability of visiting the state. Motivated by this classic result, in this work we specifically choose an exponential function of the advantages $A^\pi(s,a)=Q^\pi(s, a) - V^\pi(s)$.

\textit{Notation.} In the following we use $\sum_{s,a}$ to indicate both discrete and continuous sums (i.e., integrals) over states $s$ and actions $a$ depending on the setting. A sum with indices only, such as $\sum_{s,a}$, denotes a sum over all possible states and actions, while $\sum_{s,a\sim \mathcal{D}}$, for example, denotes a sum over sample states and actions from a batch of trajectories (the ``dataset'') $\mathcal{D}$.

==> V-MPO arXiv/content_conclusion.tex <==
\section{Conclusion}

In this work we have introduced a scalable on-policy deep reinforcement learning algorithm, V-MPO, that is applicable to both discrete and continuous control domains. For the results presented in this work neither importance weighting nor entropy regularization was used; moreover, since the size of neural network parameter updates is limited by KL constraints, we were also able to use the same learning rate for all experiments. This suggests that a scalable, performant RL algorithm may not require some of the tricks that have been developed over the past several years. Interestingly, both the original MPO algorithm for replay-based off-policy learning~\cite{Abdolmaleki2018a,Abdolmaleki2018} and V-MPO for on-policy learning are derived from similar principles, providing evidence for the benefits of this approach as an alternative to popular policy gradient-based methods.

==> V-MPO arXiv/content_experiments.tex <==
\section{Experiments}

Details on the network architecture and hyperparameters used for each task are given in Appendix~\ref{appendix:network_architecture}.

\subsection{Discrete actions: DMLab, Atari}

\begin{figure}[h]
\begin{center}
\subcaptionbox{Multi-task DMLab-30.}{\includegraphics[trim={1.5cm 0 1.2cm 0},clip,width=0.35\linewidth]{figs/dmlab30_7213230_0822_1405}}
\hspace*{0.03\columnwidth}
\subcaptionbox{Multi-task Atari-57.}{\includegraphics[trim={1.5cm 0 1.2cm 0},clip,width=0.35\columnwidth]{figs/atari57_7252372_0822_1405}}
\caption{(a) Multi-task DMLab-30. IMPALA results show 3 runs of 8 agents each; within a run hyperparameters were evolved via PBT. For V-MPO each line represents a set of hyperparameters that are fixed throughout training. The final result of R2D2+ trained for 10B environment steps on individual levels~\cite{Kapturowski2019} is also shown for comparison (orange line). (b) Multi-task Atari-57. In the IMPALA experiment, hyperparameters were evolved with PBT. For V-MPO each of the 24 lines represents a set of hyperparameters that were fixed throughout training, and all runs achieved a higher score than the best IMPALA run. Data for IMPALA (``Pixel-PopArt-IMPALA'' for DMLab-30 and ``PopArt-IMPALA'' for Atari-57) was obtained from the authors of \citeauthor{Hessel2018}~(\citeyear{Hessel2018}). Each environment frame corresponds to 4 agent steps due to the action repeat.}
\label{fig:dmlab-30}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[trim={2.1cm 0 1.2cm 0},clip,width=0.245\linewidth]{figs/dmlab_emstm_watermaze_6829056_0706_1315}
\includegraphics[trim={2.1cm 0 1.2cm 0},clip,width=0.245\linewidth]{figs/dmlab_rat_object_eat_6839137_0706_1316}
\includegraphics[trim={2.1cm 0 1.2cm 0},clip,width=0.245\linewidth]{figs/dmlab_rat_goal_doors_large_6841687_0706_1537}
\includegraphics[trim={2.1cm 0 1.2cm 0},clip,width=0.245\linewidth]{figs/dmlab_rat_object_eat_hard_6841818_0710_0236}
\caption{Example levels from DMLab-30, compared to IMPALA and more recent results from R2D2+, the larger, DMLab-specific version of R2D2~\cite{Kapturowski2019}. The IMPALA results include hyperparameter evolution with PBT.}
\label{fig:dmlab_example_levels}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[trim={1.4cm 0 1.0cm 0},clip,width=0.245\linewidth]{figs/atari_breakout_8093451_0826_0709}
\includegraphics[trim={1.4cm 0 1.0cm 0},clip,width=0.245\linewidth]{figs/atari_star_gunner_7407280_0830_0656}
\includegraphics[trim={1.4cm 0 1.0cm 0},clip,width=0.245\linewidth]{figs/atari_seaquest_7540192_0830_0658}
\includegraphics[trim={1.4cm 0 1.0cm 0},clip,width=0.245\linewidth]{figs/atari_ms_pacman_8081758_0830_0700}
\caption{Example levels from Atari. In Breakout, V-MPO achieves the maximum score of 864 in every episode. No reward clipping was applied, and the maximum length of an episode was 30 minutes (108,000 frames). Supplementary video for Ms. Pacman: \url{https://bit.ly/2lWQBy5}}
\label{fig:atari_example_levels}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\subcaptionbox{}{\includegraphics[trim={0 0 0cm 0},clip,width=0.245\linewidth]{figs/humanoid_run_7628914_0916_0334}}
\subcaptionbox{}{\includegraphics[trim={0cm 0 0cm 0},clip,width=0.245\linewidth]{figs/humanoid_gaps_8269299_0906_0553}}
%\hspace{0.25cm}\subcaptionbox{}{\includegraphics[width=0.47\linewidth]{figs/humanoid_gaps_6426357_frame}}
\subcaptionbox{}{\includegraphics[trim={0cm 0 0cm 0},clip,width=0.245\linewidth]{figs/gym_ant_v1_8454888_0916_0435}}
\subcaptionbox{}{\includegraphics[trim={0cm 0 0cm 0},clip,width=0.245\linewidth]{figs/gym_walker2d_v1_8483836_0917_0620}}

\caption{(a) Humanoid ``run'' from full state~\cite{Tassa2018} and (b) humanoid ``gaps'' from pixel observations~\cite{Merel2019}. Purple curves are the same runs but without parametric KL constraints. Det. eval.: deterministic evaluation. Supplementary video for humanoid gaps: \url{https://bit.ly/2L9KZdS}. (c)-(d) Example OpenAI Gym tasks.}
\label{fig:humanoid_gaps}
\end{center}
\end{figure}

\emph{DMLab.} DMLab-30~\cite{Beattie2016} is a collection of visually rich, partially observable 3D environments played from the first-person point of view. Like IMPALA, for DMLab we used pixel control as an auxiliary loss for representation learning~\cite{Jaderberg2016,Hessel2018}. However, we did not employ the optimistic asymmetric reward scaling used by previous IMPALA experiments to aid exploration on a subset of the DMLab levels, by weighting positive rewards more than negative rewards~\cite{Espeholt2018, Hessel2018,Kapturowski2019}. Unlike in \citeauthor{Hessel2018}~(\citeyear{Hessel2018}) we also did not use population-based training (PBT)~\cite{Jaderberg2017}. Additional details for the settings used in DMLab can be found in Table~\ref{table:dmlab_settings} of the Appendix.

Fig.~\ref{fig:dmlab-30}a shows the results for multi-task DMLab-30, comparing the V-MPO learning curves to data obtained from \citeauthor{Hessel2018}~(\citeyear{Hessel2018}) for the PopArt IMPALA agent with pixel control. We note that the result for V-MPO at 10B environment frames across all levels matches the result for the Recurrent Replay Distributed DQN (R2D2) agent~\cite{Kapturowski2019} trained on \emph{individual levels} for 10B environment steps per level. Fig.~\ref{fig:dmlab_example_levels} shows example individual levels in DMLab where V-MPO achieves scores that are substantially higher than has previously been reported, for both R2D2 and IMPALA. The pixel-control IMPALA agents shown here were carefully tuned for DMLab and are similar to the ``experts'' used in \citeauthor{Schmitt2018}~(\citeyear{Schmitt2018}); in all cases these results match or exceed previously published results for IMPALA~\cite{Espeholt2018,Kapturowski2019}.

\emph{Atari.} The Atari Learning Environment (ALE)~\cite{Bellemare2012} is a collection of 57 Atari 2600 games that has served as an important benchmark for recent deep RL methods. We used the standard preprocessing scheme and a maximum episode length of 30 minutes (108,000 frames), see Table~\ref{table:atari_settings} in the Appendix. For the multi-task setting we followed \citeauthor{Hessel2018}~(\citeyear{Hessel2018}) in setting the discount to zero on loss of life; for the example single tasks we did not employ this trick, since it can prevent the agent from achieving the highest score possible by sacrificing lives. Similarly, while in the multi-task setting we followed previous work in clipping the maximum reward to 1.0, no such clipping was applied in the single-task setting in order to preserve the original reward structure. Additional details for the settings used in Atari can be found in Table~\ref{table:atari_settings} in the Appendix.

Fig.~\ref{fig:dmlab-30}b shows the results for multi-task Atari-57, demonstrating that it is possible for a \emph{single} agent to achieve ``superhuman`` median performance on Atari-57 in approximately 4 billion ($\sim$70 million per level) environment frames.

We also compare the performance of V-MPO on a few individual Atari levels to R2D2~\cite{Kapturowski2019}, which previously achieved some of the highest scores reported for Atari. Again, V-MPO can match or exceed previously reported scores while requiring fewer interactions with the environment. In Ms. Pacman, the final performance approaches 300,000 with a 30-minute timeout (and the maximum 1M without), effectively solving the game. Inspired by the argument in \citeauthor{Kapturowski2019}~(\citeyear{Kapturowski2019}) that in a fully observable environment LSTMs enable the agent to utilize more useful representations than is available in the immediate observation, for the single-task setting we used a Transformer-XL (TrXL)~\cite{Dai2019} to replace the LSTM core. Unlike previous work for single Atari levels, we did not employ any reward clipping~\cite{Mnih2015,Espeholt2018} or nonlinear value function rescaling~\cite{Kapturowski2019}.

\subsection{Continuous control}

To demonstrate V-MPO's effectiveness in high-dimensional, continuous action spaces, here we present examples of learning to control both a simulated humanoid with 22 degrees of freedom from full state observations and one with 56 degrees of freedom from pixel observations~\cite{Tassa2018,Merel2019}. As shown in Fig.~\ref{fig:humanoid_gaps}a, for the 22-dimensional humanoid V-MPO reliably achieves higher asymptotic returns than has previously been reported, including for Deep Deterministic Policy Gradients (DDPG)~\cite{Lillicrap2015}, Stochastic Value Gradients (SVG)~\cite{Heess2015}, and MPO. These algorithms are far more sample-efficient but reach a lower final performance.

In the ``gaps'' task the 56-dimensional humanoid must run forward to match a target velocity of 4~m/s and jump over the gaps between platforms by learning to actuate joints with position-control~\cite{Merel2019}. Previously, only an agent operating in the space of pre-learned motor primitives was able to solve the task from pixel observations~\cite{Merel2018,Merel2019}; here we show that V-MPO can learn a challenging visuomotor task \emph{from scratch} (Fig.~\ref{fig:humanoid_gaps}b). For this task we also demonstrate the importance of the parametric KL constraint, without which the agent learns poorly.

In Figs.~\ref{fig:humanoid_gaps}c-d we also show that V-MPO achieves the highest asymptotic performance reported for two OpenAI Gym tasks~\cite{Brockman2016}. Again, MPO and Stochastic Actor-Critic~\cite{Haarnoja2018} are far more sample-efficient but reach a lower final performance.


==> V-MPO arXiv/content_introduction.tex <==
\section{Introduction}
\label{introduction}

Deep reinforcement learning (RL) with neural network function approximators has achieved superhuman performance in several challenging domains~\cite{Mnih2015,Silver2016,Silver2018}. Some of the most successful recent applications of deep RL to difficult environments such as Dota~2~\cite{OpenAI2018}, Capture the Flag~\cite{Jaderberg2019}, Starcraft~II~\cite{DeepMind2019}, and dexterous object manipulation~\cite{OpenAI2018a} have used policy gradient-based methods such as Proximal Policy Optimization (PPO)~\cite{Schulman2017} and the Importance-Weighted Actor-Learner Architecture (IMPALA)~\cite{Espeholt2018}, both in the approximately on-policy setting.

Policy gradients, however, can suffer from large variance that may limit performance, especially for high-dimensional action spaces~\cite{Wu2018}. In practice, moreover, policy gradient methods typically employ carefully tuned entropy regularization in order to prevent policy collapse. As an alternative to policy gradient-based algorithms, in this work we introduce an approximate policy iteration algorithm that adapts Maximum a Posteriori Policy Optimization (MPO)~\cite{Abdolmaleki2018a,Abdolmaleki2018} to the on-policy setting. The modified algorithm, V-MPO, relies on a learned state-value function $V(s)$ instead of the state-action value function used in MPO. Like MPO, rather than directly updating the parameters in the direction of the policy gradient, V-MPO first constructs a target distribution for the policy update subject to a sample-based KL constraint, then calculates the gradient that partially moves the parameters toward that target, again subject to a KL constraint.

As we are particularly interested in scalable RL algorithms that can be applied to multi-task settings where a single agent must perform a wide variety of tasks, we show for the case of discrete actions that the proposed algorithm surpasses previously reported performance in the multi-task setting for both the Atari-57~\cite{Bellemare2012} and DMLab-30~\cite{Beattie2016} benchmark suites, and does so reliably without population-based tuning of hyperparameters~\cite{Jaderberg2017}. For a few individual levels in DMLab and Atari we also show that V-MPO can achieve scores that are substantially higher than has previously been reported, especially in the challenging Ms. Pacman.

V-MPO is also applicable to problems with high-dimensional, continuous action spaces. We demonstrate this in the context of learning to control both a 22-dimensional simulated humanoid from full state observations---where V-MPO reliably achieves higher asymptotic performance than previous algorithms---and a 56-dimensional simulated humanoid from pixel observations~\cite{Tassa2018,Merel2019}. In addition, for several OpenAI Gym tasks~\cite{Brockman2016} we show that V-MPO achieves higher asymptotic performance than has previously been reported.


==> V-MPO arXiv/content_method.tex <==
\section{Method}

V-MPO is an approximate policy iteration~\cite{Sutton1998} algorithm with a specific prescription for the policy improvement step. In general, policy iteration uses the fact that the true state-value function $V^\pi$ corresponding to policy $\pi$ can be used to obtain an improved policy $\pi'$. Thus we can

\begin{enumerate}
    \item Generate trajectories $\tau$ from an old ``target'' policy $\pi_{\theta_\text{old}}(a|s)$ whose parameters $\theta_\text{old}$ are fixed. To control the amount of data generated by a particular policy, we use a target network which is fixed for $T_\text{target}$ learning steps (Fig.~\ref{fig:schematic}a in the Appendix).
    \item Evaluate the policy $\pi_{\theta_\text{old}}(a|s)$ by learning the value function $V^{\pi_{\theta_\text{old}}}(s)$ from empirical returns and estimating the corresponding advantages $A^{\pi_{\theta_\text{old}}}(s,a)$ for the actions that were taken.
    \item Estimate an improved ``online'' policy $\pi_\theta(a|s)$ based on $A^{\pi_{\theta_\text{old}}}(s,a)$.
\end{enumerate}

The first two steps are standard, and describing V-MPO's approach to step (3) is the essential contribution of this work. At a high level, our strategy is to first construct a nonparametric target distribution for the policy update, then partially move the parametric policy towards this distribution subject to a KL constraint. Ultimately, we use gradient descent to optimize a single, relatively simple loss, which we provide here in complete form in order to ground the derivation of the algorithm.

Consider a batch of data $\mathcal{D}$ consisting of a number of trajectories, with $|\mathcal{D}|$ total state-action samples. Each trajectory consists of an unroll of length $n$ of the form $\tau=\big[ (s_t,a_t,r_{t+1}), \ldots, (s_{t+n-1},a_{t+n-1},r_{t+n}),\ s_{t+n} \big]$ including the bootstrapped state $s_{t+n}$, where $r_{t+1}=r(s_t,a_t)$. The total loss is the sum of a policy evaluation loss and a policy improvement loss,
\begin{equation}
   \mathcal{L}(\phi, \theta, \eta, \alpha) = \mathcal{L}_V(\phi) + \mathcal{L}_\text{V-MPO}(\theta, \eta, \alpha), \label{eq:total_loss}
\end{equation} where $\phi$ are the parameters of the value network, $\theta$ the parameters of the policy network, and $\eta$ and $\alpha$ are Lagrange multipliers. In practice, the policy and value networks share most of their parameters in the form of a shared convolutional network (a ResNet) and recurrent LSTM core, and are optimized together (Fig.~\ref{fig:schematic}b in the Appendix)~\cite{Mnih2016}. We note, however, that the value network parameters $\phi$ are considered fixed for the policy improvement loss, and gradients are not propagated.

The policy evaluation loss for the value function, $\mathcal{L}_V(\phi)$, is the standard regression to $n$-step returns and is given by Eq.~\ref{eq:value_loss} below. The policy improvement loss $\mathcal{L}_\text{V-MPO}(\theta, \eta, \alpha)$ is given by
\begin{equation}
    \mathcal{L}_\text{V-MPO}(\theta, \eta, \alpha) = \mathcal{L}_\pi(\theta) + \mathcal{L}_\eta(\eta) + \mathcal{L}_\alpha(\theta,\alpha).
\end{equation} Here the policy loss is the weighted maximum likelihood loss
\begin{equation}
    \mathcal{L}_\pi(\theta) = -\sum_{s,a\sim \tilde{\mathcal{D}}} \psi(s,a) \log \pi_\theta(a|s), \qquad 
    \psi(s,a) = \frac{\exp \big( \frac{A^\text{target}(s,a)}{\eta} \big)}{\sum_{s,a\sim \tilde{\mathcal{D}}} \exp \big( \frac{A^\text{target}(s,a)}{\eta} \big)}, \label{eq:policy_loss}
\end{equation} where the advantages $A^\text{target}(s,a)$ for the target network policy $\pi_{\theta_\text{target}}(a|s)$ are estimated according to the standard method described below. The tilde over the dataset, $\tilde{\mathcal{D}}$, indicates that we take samples corresponding to the top half advantages in the batch of data. The $\eta$, or ``temperature'', loss is
\begin{equation}
    \mathcal{L}_\eta(\eta) = \eta \epsilon_\eta + \eta \log \Bigg[ \frac{1}{|\tilde{\mathcal{D}}|}\sum_{s,a\sim \tilde{\mathcal{D}}} \exp\bigg( \frac{A^\text{target}(s,a)}{\eta} \bigg) \Bigg]. \label{eq:L_eta}
\end{equation} The KL constraint, which can be viewed as a form of trust-region loss, is given by
\begin{align}
    &\mathcal{L}_\alpha(\theta,\alpha)
    = \frac{1}{|\mathcal{D}|}\sum_{s \in \mathcal{D}} \Big[  \alpha \big( \epsilon_\alpha - \stopgradient\big[\big[ D_\text{KL}\big( \pi_{\theta_\text{target}}(a|s) \| \pi_{\vphantom{\theta_\text{target}}\theta}(a|s) \big) \big]\big] \Big) + \stopgradient[[\alpha]] D_\text{KL}\big( \pi_{\theta_\text{target}}(a|s) \| \pi_{\vphantom{\theta_\text{old}}\theta}(a|s) \big) \Big], \label{eq:L_alpha}
\end{align} where $\stopgradient[[\cdot]]$ indicates a stop gradient, i.e., that the enclosed term is assumed constant with respect to all variables. Note that here we use the full batch $\mathcal{D}$, not $\tilde{\mathcal{D}}$.

We used the Adam optimizer~\cite{Kingma2015} with default TensorFlow hyperparameters to optimize the total loss in Eq.~\ref{eq:total_loss}. In particular, the learning rate was fixed at $10^{-4}$ for all experiments.

%-------------------------------------------------------------------------------
% Subsection.
%-------------------------------------------------------------------------------

\subsection{Policy evaluation}

In the present setting, policy evaluation means learning an approximate state-value function $V^\pi(s)$ given a policy $\pi(a|s)$, which we keep fixed for $T_\text{target}$ learning steps (i.e., batches of trajectories). We note that the value function corresponding to the target policy is instantiated in the ``online'' network receiving gradient updates; bootstrapping uses the online value function, as it is the best available estimate of the value function for the target policy. Thus in this section $\pi$ refers to $\pi_{\theta_\text{old}}$, while the value function update is performed on the current $\phi$, which may share parameters with the current $\theta$.

We fit a parametric value function $V^\pi_\phi(s)$ with parameters $\phi$ by minimizing the squared loss
\begin{align}
    \mathcal{L}_V(\phi) 
    &= \frac{1}{2|\mathcal{D}|}\sum_{s_t \sim \mathcal{D}} \big( V^\pi_\phi(s_t) - G^{(n)}_t \big)^2, \label{eq:value_loss}
\end{align} where $G^{(n)}_t$ is the standard $n$-step target for the value function at state $s_t$ at time $t$~\cite{Sutton1998}. This return uses the actual rewards in the trajectory and bootstraps from the value function for the rest: for each $\ell=t,\ldots,t+n-1$ in an unroll, $G^{(n)}_\ell = \sum_{k=\ell}^{t+n-1} \gamma^{k-\ell}r_k + \gamma^{t+n-\ell} V^\pi_\phi(s_{t+n})$. 
The advantages, which are the key quantity of interest for the policy improvement step in V-MPO, are then given by $A^\pi(s_t,a_t) = G^{(n)}_t - V^\pi_\phi(s_t)$ for each $s_t,a_t$ in the batch of trajectories.

\emph{PopArt normalization.} As we are interested in the multi-task setting where a single agent must learn a large number of tasks with differing reward scales, we used PopArt~\cite{Hasselt2016,Hessel2018} for the value function, even when training on a single task. Specifically, the value function outputs a separate value for each task in normalized space, which is converted to actual returns by a shift and scaling operation, the statistics of which are learned during training. We used a scale lower bound of $10^{-2}$, scale upper bound of $10^6$, and learning rate of $10^{-4}$ for the statistics. The lower bound guards against numerical issues when rewards are extremely sparse.

\emph{Importance-weighting for off-policy data.} It is possible to importance-weight the samples using V-trace to correct for off-policy data~\cite{Espeholt2018}, for example when data is taken from a replay buffer. For simplicity, however, no importance-weighting was used for the experiments presented in this work, which were mostly on-policy.

%-------------------------------------------------------------------------------
% Subsection.
%-------------------------------------------------------------------------------

\subsection{Policy improvement in V-MPO}

In this section we show how, given the advantage function $A^{\pi_{\theta_\text{old}}}(s,a)$ for the state-action distribution $p_{\theta_\text{old}}(s,a)=\pi_{\theta_\text{old}}(a|s)p(s)$ induced by the old policy $\pi_{\theta_\text{old}}(a|s)$, we can estimate an improved policy $\pi_\theta(a|s)$. More formally, let $\mathcal{I}$ denote the binary event that the new policy is an improvement (in a sense to be defined below) over the previous policy: $\mathcal{I}=1$ if the policy is successfully improved and 0 otherwise. Then we would like to find the mode of the posterior distribution over parameters $\theta$ conditioned on this event, i.e., we seek the maximum a posteriori (MAP) estimate
\begin{equation}
    \theta^* = \operatorname{arg} \max_{\theta} \big[ \log p_{\theta}(\mathcal{I}=1) + \log p(\theta) \big], \label{eq:map_estimate}
\end{equation} where we have written $p(\mathcal{I}=1|\theta)$ as $p_\theta(\mathcal{I}=1)$ to emphasize the parametric nature of the dependence on $\theta$. We use the well-known identity $\log p(X) = \mathbb{E}_{\psi(Z)} \big[ \log \frac{p(X,Z)}{\psi(Z)} \big] + D_\text{KL}\big( \psi(Z) \| p(Z|X) \big)$ for any latent distribution $\psi(Z)$, where $D_\text{KL}(\psi(Z)\|p(Z|X))$ is the Kullback-Leibler divergence between $\psi(Z)$ and $p(Z|X)$ with respect to $Z$, and the first term is a lower bound because the KL divergence is always non-negative. Then considering $s,a$ as latent variables,
\begin{equation}
    \log p_\theta(\mathcal{I}=1) = \sum_{s,a} \psi(s,a) \log \frac{p_\theta(\mathcal{I}=1,s,a)}{\psi(s,a)} + D_\text{KL}\big( \psi(s,a) \| p_\theta(s,a|\mathcal{I}=1) \big). \label{eq:elbo}
\end{equation}

Policy improvement in V-MPO consists of the following two steps which have direct correspondences to the expectation maximization (EM) algorithm~\cite{Neal1998}: In the expectation (E) step, we choose the variational distribution $\psi(s,a)$ such that the lower bound on $\log p_\theta(\mathcal{I}=1)$ is as tight as possible, by minimizing the KL term. In the maximization (M) step we then find parameters $\theta$ that maximize the corresponding lower bound, together with the prior term in Eq.~\ref{eq:map_estimate}.

%-------------------------------------------------------------------------------
% Subsection.
%-------------------------------------------------------------------------------

\subsubsection{E-step}

In the E-step, our goal is to choose the variational distribution $\psi(s,a)$ such that the lower bound on $\log p_\theta(\mathcal{I}=1)$ is as tight as possible, which is the case when the KL term in Eq.~\ref{eq:elbo} is zero. Given the old parameters $\theta_\text{old}$, this simply leads to $\psi(s,a) = p_{\theta_\text{old}}(s,a|\mathcal{I}=1)$, or
\begin{equation}
    \psi(s,a) = \frac{p_{\theta_\text{old}}(s,a)p_{\theta_\text{old}}(\mathcal{I}=1|s,a)}{p_{\theta_\text{old}}(\mathcal{I}=1)}, \qquad p_{\theta_\text{old}}(\mathcal{I}=1) = \sum_{s,a} p_{\theta_\text{old}}(s,a)p_{\theta_\text{old}}(\mathcal{I}=1|s,a). \label{eq:psi_general}
\end{equation} Intuitively, this solution weights the probability of each state-action pair with its relative improvement probability $p_{\theta_\text{old}}(\mathcal{I}=1|s,a)$. We now choose a distribution $p_{\theta_\text{old}}(\mathcal{I}=1|s,a)$ that leads to our desired outcome. As we prefer actions that lead to a higher advantage in each state, we suppose that this probability is given by
\begin{equation}
    p_{\theta_\text{old}}(\mathcal{I}=1|s,a) \propto \exp \bigg( \frac{A^{\pi_{\theta_\text{old}}}(s,a)}{\eta} \bigg) \label{eq:improvement_criterion}
\end{equation} for some temperature $\eta > 0$, from which we obtain the equation on the right in Eq.~\ref{eq:policy_loss}. This probability depends on the \emph{old} parameters $\theta_\text{old}$ and not on the new parameters $\theta$. Meanwhile, the value of $\eta$ allows us to control the diversity of actions that contribute to the weighting, but at the moment is arbitrary. It turns out, however, that we can tune $\eta$ as part of the optimization, which is desirable since the optimal value of $\eta$ changes across iterations. The convex loss that achieves this, Eq.~\ref{eq:L_eta}, is derived in Appendix~\ref{appendix:temperature_loss} by minimizing the KL term in Eq.~\ref{eq:elbo} subject to a hard constraint on $\psi(s,a)$.

\emph{Top-$k$ advantages.} We found that learning improves substantially if we take only the samples corresponding to the highest 50\% of advantages in each batch for the E-step, corresponding to the use of $\tilde{\mathcal{D}}$ rather than $\mathcal{D}$ in Eqs.~\ref{eq:policy_loss},~\ref{eq:L_eta}. Importantly, these must be consistent between the maximum likelihood weights in Eq.~\ref{eq:policy_loss} and the temperature loss in Eq.~\ref{eq:L_eta}, since, mathematically, this is justified by choosing the corresponding policy improvement probability in Eq.~\ref{eq:improvement_criterion} to only use the top half of the advantages. This is similar to the technique used in Covariance Matrix Adaptation - Evolutionary Strategy (CMA-ES)~\cite{Hansen1997,Abdolmaleki2017}, and is a special case of the more general feature that any rank-preserving transformation is allowed under this formalism.

\emph{Importance weighting for off-policy corrections.} As for the value function, importance weights can be used in the policy improvement step to correct for off-policy data. While not used for the experiments presented in this work, details for how to carry out this correction are given in Appendix~\ref{appendix:importance_weighting}.

%-------------------------------------------------------------------------------
% Subsection.
%-------------------------------------------------------------------------------

\subsubsection{M-step: Constrained supervised learning of the parametric policy}

In the E-step we found the nonparametric variational state-action distribution $\psi(s,a)$, Eq.~\ref{eq:psi_general}, that gives the tightest lower bound to $p_\theta(\mathcal{I}=1)$ in Eq.~\ref{eq:elbo}. In the M-step we maximize this lower bound together with the prior term $\log p(\theta)$ with respect to the parameters $\theta$, which effectively leads to a constrained weighted maximum likelihood problem. Thus the introduction of the nonparametric distribution in Eq.~\ref{eq:psi_general} separates the RL procedure from the neural network fitting.

We would like to find new parameters $\theta$ that minimize
\begin{equation}
    \mathcal{L}(\theta) 
    = -\sum_{s,a} \psi(s,a) \log \frac{p_\theta(\mathcal{I}=1,s,a)}{\psi(s,a)} - \log p(\theta). \label{eq:original_m_step_loss}
\end{equation} Note, however, that so far we have worked with the joint state-action distribution $\psi(s,a)$ while we are in fact optimizing for the policy, which is the conditional distribution $\pi_\theta(a|s)$. Writing $p_\theta(s,a) = \pi_\theta(a|s)p(s)$ since only the policy is parametrized by $\theta$ and dropping terms that are not parametrized by $\theta$, the first term of Eq.~\ref{eq:original_m_step_loss} is seen to be the weighted maximum likelihood policy loss
\begin{equation}
   \mathcal{L}_\pi(\theta) = -\sum_{s,a} \psi(s,a) \log \pi_\theta(a|s).
\end{equation} In the sample-based computation of this loss, we assume that any state-action pairs not in the batch of trajectories have zero weight, leading to the normalization in Eq.~\ref{eq:policy_loss}.

As in the original MPO algorithm, a useful prior is to keep the new policy $\pi_\theta(a|s)$ close to the old policy $\pi_{\theta_\text{old}}(a|s)$: $\log p(\theta) \approx -\alpha \mathbb{E}_{s\sim p(s)} \big[ \dkl\big( \pi_{\theta_\text{old}}(a|s) \| \pi_{\vphantom{\theta_\text{old}}\theta}(a|s) \big) \big]$. While intuitive, we motivate this more formally in Appendix~\ref{appendix:kl-constraint}. It is again more convenient to specify a bound on the KL divergence instead of tuning $\alpha$ directly, so we solve the constrained optimization problem
\begin{equation}
    \theta^* = \argmin{\theta} - \sum_{s,a} \psi(s,a) \log \pi_{\theta}(a|s) \quad \text{s.t. } \operatornamewithlimits{\mathbb{E}}_{s\sim p(s)} \Big[ D_\text{KL}\big( \pi_{\theta_\text{old}}(a|s) \| \pi_\theta(a|s) \big) \Big] < \epsilon_\alpha. \label{eq:m_step_constraint}
\end{equation} Intuitively, the constraint in the E-step expressed by Eq.~\ref{eq:e_step_constraint} in Appendix~\ref{appendix:temperature_loss} for tuning the temperature only constrains the nonparametric distribution; it is the constraint in Eq.~\ref{eq:m_step_constraint} that directly limits the change in the parametric policy, in particular for states and actions that were not in the batch of samples and which rely on the generalization capabilities of the neural network function approximator.

To make the constrained optimization problem amenable to gradient descent, we use Lagrangian relaxation to write the unconstrained objective as
\begin{equation}
    \mathcal{J}(\theta, \alpha)
    = \mathcal{L}_\pi(\theta) + \alpha \bigg( \epsilon_\alpha - \operatornamewithlimits{\mathbb{E}}_{s\sim p(s)} \Big[ D_\text{KL} \big( \pi_{\theta_\text{old}}(a|s) \| \pi_{\vphantom{\theta_\text{old}}\theta}(a|s) \big) \Big] \bigg), \label{eq:m_step_objective}
\end{equation} which we can optimize by following a coordinate-descent strategy, alternating between the optimization over $\theta$ and $\alpha$. Thus, in addition to the policy loss we arrive at the constraint loss
\begin{equation}
    \mathcal{L}_\alpha(\theta,\alpha) = \alpha \bigg( \epsilon_\alpha - \operatornamewithlimits{\mathbb{E}}_{s\sim p(s)} \Big[ \stopgradient\big[\big[ D_\text{KL}\big( \pi_{\theta_\text{old}} \| \pi_{\vphantom{\theta_\text{old}}\theta} \big) \big]\big] \Big] \bigg) + \stopgradient[[\alpha]] \operatornamewithlimits{\mathbb{E}}_{s\sim p(s)} \Big[ D_\text{KL}\big( \pi_{\theta_\text{old}} \| \pi_{\vphantom{\theta_\text{old}}\theta} \big) \Big]. \label{eq:m_step_kl_constraint}
\end{equation} Replacing the sum over states with samples gives Eq.~\ref{eq:L_alpha}. Since $\eta$ and $\alpha$ are Lagrange multipliers that must be positive, after each gradient update we project the resulting $\eta$ and $\alpha$ to a small positive value which we choose to be $\eta_\text{min}=\alpha_\text{min}=10^{-8}$ throughout the results presented below.

For continuous action spaces parametrized by Gaussian distributions, we use decoupled KL constraints for the M-step in Eq.~\ref{eq:m_step_kl_constraint} as in \citeauthor{Abdolmaleki2018}~(\citeyear{Abdolmaleki2018}); the precise form is given in Appendix~\ref{appendix:continuous_control}.



==> V-MPO arXiv/content_related_work.tex <==
\section{Related work}

V-MPO shares many similarities, and thus relevant related work, with the original MPO algorithm~\cite{Abdolmaleki2018a,Abdolmaleki2018}. In particular, the general idea of using KL constraints to limit the size of policy updates is present in both Trust Region Policy Optimization (TRPO; \citeauthor{Schulman2015a}, \citeyear{Schulman2015a}) and Proximal Policy Optimization (PPO)~\cite{Schulman2017}; we note, however, that this corresponds to the E-step constraint in V-MPO. Meanwhile, the introduction of the M-step KL constraint and the use of top-$k$ advantages distinguishes V-MPO from Relative Entropy Policy Search (REPS)~\cite{Peters2008a}. Interestingly, previous attempts to use REPS with neural network function approximators reported very poor performance, being particularly prone to local optima~\cite{Duan2018}. In contrast, we find that the principles of EM-style policy optimization, when combined with appropriate constraints, can reliably train powerful neural networks, including transformers, for RL tasks.

Like V-MPO, Supervised Policy Update (SPU)~\cite{Vuong2018} seeks to exactly solve an optimization problem and fit the parametric policy to this solution. As we argue in Appendix~\ref{appendix:spu}, however, SPU uses this nonparametric distribution quite differently from V-MPO; as a result, the final algorithm is closer to a policy gradient algorithm such as PPO.

==> V-MPO arXiv/latex_macros_iclr2020.tex <==
\renewcommand{\d}{\partial}
\newcommand{\der}[2]{\frac{d#1}{d#2}}
\newcommand{\ders}[2]{\frac{d^2#1}{d#2^2}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pders}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pdersmixed}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\br}[1]{\underline{#1}}
\newcommand{\lp}{\bigg(}
\renewcommand{\rp}{\bigg)}
\newcommand{\Lp}{\Bigg(}
\newcommand{\Rp}{\Bigg)}
\newcommand{\lb}{\bigg[}
\renewcommand{\rb}{\bigg]}
\newcommand{\Lb}{\Bigg[}
\newcommand{\Rb}{\Bigg]}
\newcommand{\lc}{\bigg\{}
\renewcommand{\rc}{\bigg\}}
\newcommand{\Lc}{\Bigg\{}
\newcommand{\Rc}{\Bigg\}}
\newcommand{\pf}[2]{\lp\frac{#1}{#2}\rp}
\newcommand{\sqrtfrac}[2]{\sqrt{\frac{#1}{#2}}}

\let\oldvec\vec
\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\braket}[2]{\langle#1|#2\rangle}
\newcommand{\mean}[1]{\langle#1\rangle}
\newcommand{\Mean}[1]{\big\langle #1 \big\rangle}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\colv}[2]{\left(\begin{matrix} #1 \\ #2 \end{matrix}\right)}
\newcommand{\rowv}[2]{\left(\begin{matrix} #1 & #2 \end{matrix}\right)}
\newcommand{\mat}[4]{\left(\begin{matrix} #1 & #2 \\ #3 & #4 \end{matrix}\right)}
\newcommand{\sinc}{\operatorname{sinc}}
\newcommand{\sech}{\operatorname{sech}}
\newcommand{\Si}{\operatorname{Si}}
\renewcommand{\re}{\operatorname{Re}}
\newcommand{\im}{\operatorname{Im}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}
\newcommand{\erfi}{\operatorname{erfi}}
\newcommand{\sgn}{\operatorname{sgn}}

\renewcommand{\sigmoid}{\operatorname{sigmoid}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\unit}[1]{\text{ #1}}

\newcommand{\var}{\operatorname{Var}}
\newcommand{\cov}{\operatorname{Cov}}

%\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\maxover}{\operatornamewithlimits{max}}

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\renewcommand{\argmax}[1]{\operatorname{arg}\operatornamewithlimits{max}_{#1}}
\renewcommand{\argmin}[1]{\operatorname{arg}\operatornamewithlimits{min}_{#1}}

\newcommand{\stopgradient}{\operatorname{sg}}

\newcommand{\dkl}{D_\text{KL}}
\newcommand{\expectation}[1]{\operatornamewithlimits{\mathbb{E}}_{#1}}

% Probability
%\DeclareMathOperator{\E}{$\mathbb{E}$}

==> V-MPO arXiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

